The Natural Language of Actions

We introduce Act2Vec, a general framework for learning context-based action representation for Reinforcement Learning. Representing actions in a vector space help reinforcement learning algorithms achieve better performance by grouping similar actions and utilizing relations between different actions. We show how prior knowledge of an environment can be extracted from demonstrations and injected into action vector representations that encode natural compatible behavior. We then use these for augmenting state representations as well as improving function approximation of Q-values. We visualize and test action embeddings in three domains including a drawing task, a high dimensional navigation task, and the large action space domain of StarCraft II.

==> ms <==
\begin{thebibliography}{34}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Abbeel \& Ng(2004)Abbeel and Ng]{thm1_ref}
Abbeel, P. and Ng, A.~Y.
\newblock Apprenticeship learning via inverse reinforcement learning.
\newblock In \emph{Proceedings of the twenty-first international conference on
  Machine learning}, pp.\ ~1. ACM, 2004.

\bibitem[Argall et~al.(2009)Argall, Chernova, Veloso, and Browning]{imitation3}
Argall, B.~D., Chernova, S., Veloso, M., and Browning, B.
\newblock A survey of robot learning from demonstration.
\newblock \emph{Robotics and autonomous systems}, 57\penalty0 (5):\penalty0
  469--483, 2009.

\bibitem[Beattie et~al.(2016)Beattie, Leibo, Teplyashin, Ward, Wainwright,
  K{\"u}ttler, Lefrancq, Green, Vald{\'e}s, Sadik, et~al.]{deepmind_lab}
Beattie, C., Leibo, J.~Z., Teplyashin, D., Ward, T., Wainwright, M.,
  K{\"u}ttler, H., Lefrancq, A., Green, S., Vald{\'e}s, V., Sadik, A., et~al.
\newblock Deepmind lab.
\newblock \emph{arXiv preprint arXiv:1612.03801}, 2016.

\bibitem[Caruana(1997)]{multi-task1}
Caruana, R.
\newblock Multitask learning.
\newblock \emph{Machine learning}, 28\penalty0 (1):\penalty0 41--75, 1997.

\bibitem[Chandak et~al.(2019)Chandak, Theocharous, Kostas, Jordan, and
  Thomas]{chandak2019learning}
Chandak, Y., Theocharous, G., Kostas, J., Jordan, S., and Thomas, P.~S.
\newblock Learning action representations for reinforcement learning.
\newblock \emph{arXiv preprint arXiv:1902.00183}, 2019.

\bibitem[Cheema et~al.(2012)Cheema, Gulwani, and LaViola]{quickdraw}
Cheema, S., Gulwani, S., and LaViola, J.
\newblock Quickdraw: improving drawing experience for geometric diagrams.
\newblock In \emph{Proceedings of the SIGCHI Conference on Human Factors in
  Computing Systems}, pp.\  1037--1064. ACM, 2012.

\bibitem[Daniel et~al.(2012)Daniel, Neumann, and Peters]{skill-entropy1}
Daniel, C., Neumann, G., and Peters, J.
\newblock Hierarchical relative entropy policy search.
\newblock In \emph{Artificial Intelligence and Statistics}, pp.\  273--281,
  2012.

\bibitem[Dulac-Arnold et~al.(2015)Dulac-Arnold, Evans, van Hasselt, Sunehag,
  Lillicrap, Hunt, Mann, Weber, Degris, and Coppin]{dulac2015deep}
Dulac-Arnold, G., Evans, R., van Hasselt, H., Sunehag, P., Lillicrap, T., Hunt,
  J., Mann, T., Weber, T., Degris, T., and Coppin, B.
\newblock Deep reinforcement learning in large discrete action spaces.
\newblock \emph{arXiv preprint arXiv:1512.07679}, 2015.

\bibitem[End et~al.(2017)End, Akrour, Peters, and Neumann]{skill-entropy2}
End, F., Akrour, R., Peters, J., and Neumann, G.
\newblock Layered direct policy search for learning hierarchical skills.
\newblock In \emph{Robotics and Automation (ICRA), 2017 IEEE International
  Conference on}, pp.\  6442--6448. IEEE, 2017.

\bibitem[Engel \& Mannor(2001)Engel and Mannor]{hemp}
Engel, Y. and Mannor, S.
\newblock Learning embedded maps of markov processes.
\newblock In \emph{in Proceedings of ICML 2001}. Citeseer, 2001.

\bibitem[Firth(1957)]{word_contex_idea}
Firth, J.~R.
\newblock A synopsis of linguistic theory, 1930-1955.
\newblock \emph{Studies in linguistic analysis}, 1957.

\bibitem[Gabriel et~al.(2017)Gabriel, Akrour, Peters, and
  Neumann]{skill-entropy3}
Gabriel, A., Akrour, R., Peters, J., and Neumann, G.
\newblock Empowered skills.
\newblock In \emph{Robotics and Automation (ICRA), 2017 IEEE International
  Conference on}, pp.\  6435--6441. IEEE, 2017.

\bibitem[Goodfellow et~al.()Goodfellow, Bengio, Courville, and
  Bengio]{representation}
Goodfellow, I., Bengio, Y., Courville, A., and Bengio, Y.
\newblock \emph{Deep learning}, volume~1.

\bibitem[Gupta et~al.(2017)Gupta, Devin, Liu, Abbeel, and Levine]{transfer3}
Gupta, A., Devin, C., Liu, Y., Abbeel, P., and Levine, S.
\newblock Learning invariant feature spaces to transfer skills with
  reinforcement learning.
\newblock \emph{ICLR}, 2017.

\bibitem[Hausman et~al.()Hausman, Springenberg, Wang, Heess, and
  Riedmiller]{skill-embedding2}
Hausman, K., Springenberg, J.~T., Wang, Z., Heess, N., and Riedmiller, M.
\newblock Learning an embedding space for transferable robot skills.
\newblock \emph{ICLR}.

\bibitem[He et~al.(2016)He, Chen, He, Gao, Li, Deng, and Ostendorf]{nlp_rl}
He, J., Chen, J., He, X., Gao, J., Li, L., Deng, L., and Ostendorf, M.
\newblock Deep reinforcement learning with a natural language action space.
\newblock In \emph{Proceedings of the 54th Annual Meeting of the Association
  for Computational Linguistics (Volume 1: Long Papers)}, volume~1, pp.\
  1621--1630, 2016.

\bibitem[Kroemer \& Sukhatme(2016)Kroemer and Sukhatme]{skill-embedding3}
Kroemer, O. and Sukhatme, G.~S.
\newblock Learning relevant features for manipulation skills using meta-level
  priors.
\newblock \emph{arXiv preprint arXiv:1605.04439}, 2016.

\bibitem[Levy \& Goldberg(2014)Levy and Goldberg]{PPMI_SGNS}
Levy, O. and Goldberg, Y.
\newblock Neural word embedding as implicit matrix factorization.
\newblock In \emph{Advances in neural information processing systems}, pp.\
  2177--2185, 2014.

\bibitem[Littman \& Sutton(2002)Littman and Sutton]{psr}
Littman, M.~L. and Sutton, R.~S.
\newblock Predictive representations of state.
\newblock In \emph{Advances in neural information processing systems}, pp.\
  1555--1561, 2002.

\bibitem[Maaten \& Hinton(2008)Maaten and Hinton]{tsne}
Maaten, L. v.~d. and Hinton, G.
\newblock Visualizing data using t-sne.
\newblock \emph{Journal of machine learning research}, 9\penalty0
  (Nov):\penalty0 2579--2605, 2008.

\bibitem[Mikolov et~al.(2013{\natexlab{a}})Mikolov, Chen, Corrado, and
  Dean]{skip_gram}
Mikolov, T., Chen, K., Corrado, G., and Dean, J.
\newblock Efficient estimation of word representations in vector space.
\newblock \emph{arXiv preprint arXiv:1301.3781}, 2013{\natexlab{a}}.

\bibitem[Mikolov et~al.(2013{\natexlab{b}})Mikolov, Sutskever, Chen, Corrado,
  and Dean]{word2vec}
Mikolov, T., Sutskever, I., Chen, K., Corrado, G.~S., and Dean, J.
\newblock Distributed representations of words and phrases and their
  compositionality.
\newblock In \emph{Advances in neural information processing systems}, pp.\
  3111--3119, 2013{\natexlab{b}}.

\bibitem[Mnih et~al.(2015)Mnih, Kavukcuoglu, Silver, Rusu, Veness, Bellemare,
  Graves, Riedmiller, Fidjeland, Ostrovski, et~al.]{dqn}
Mnih, V., Kavukcuoglu, K., Silver, D., Rusu, A.~A., Veness, J., Bellemare,
  M.~G., Graves, A., Riedmiller, M., Fidjeland, A.~K., Ostrovski, G., et~al.
\newblock Human-level control through deep reinforcement learning.
\newblock \emph{Nature}, 518\penalty0 (7540):\penalty0 529, 2015.

\bibitem[Pastor et~al.(2012)Pastor, Kalakrishnan, Righetti, and
  Schaal]{skill-embedding1}
Pastor, P., Kalakrishnan, M., Righetti, L., and Schaal, S.
\newblock Towards associative skill memories.
\newblock In \emph{Humanoid Robots (Humanoids), 2012 12th IEEE-RAS
  International Conference on}, pp.\  309--315. IEEE, 2012.

\bibitem[Pennington et~al.(2014)Pennington, Socher, and Manning]{glove}
Pennington, J., Socher, R., and Manning, C.
\newblock Glove: Global vectors for word representation.
\newblock In \emph{Proceedings of the 2014 conference on empirical methods in
  natural language processing (EMNLP)}, pp.\  1532--1543, 2014.

\bibitem[Ruder(2017)]{multi-task2}
Ruder, S.
\newblock An overview of multi-task learning in deep neural networks.
\newblock \emph{arXiv preprint arXiv:1706.05098}, 2017.

\bibitem[Sapir(1921)]{language_intro}
Sapir, E.
\newblock \emph{An introduction to the study of speech}.
\newblock Citeseer, 1921.

\bibitem[Schaal(1997)]{imitation2}
Schaal, S.
\newblock Learning from demonstration.
\newblock In \emph{Advances in neural information processing systems}, pp.\
  1040--1046, 1997.

\bibitem[Schaal(1999)]{imitation1}
Schaal, S.
\newblock Is imitation learning the route to humanoid robots?
\newblock \emph{Trends in cognitive sciences}, 3\penalty0 (6):\penalty0
  233--242, 1999.

\bibitem[Schulman et~al.(2017)Schulman, Wolski, Dhariwal, Radford, and
  Klimov]{ppo}
Schulman, J., Wolski, F., Dhariwal, P., Radford, A., and Klimov, O.
\newblock Proximal policy optimization algorithms.
\newblock \emph{arXiv preprint arXiv:1707.06347}, 2017.

\bibitem[Taylor \& Stone(2009{\natexlab{a}})Taylor and Stone]{transfer1}
Taylor, M.~E. and Stone, P.
\newblock Transfer learning for reinforcement learning domains: A survey.
\newblock \emph{Journal of Machine Learning Research}, 10\penalty0
  (Jul):\penalty0 1633--1685, 2009{\natexlab{a}}.

\bibitem[Taylor \& Stone(2009{\natexlab{b}})Taylor and Stone]{transfer2}
Taylor, M.~E. and Stone, P.
\newblock Transfer learning for reinforcement learning domains: A survey.
\newblock \emph{Journal of Machine Learning Research}, 10\penalty0
  (Jul):\penalty0 1633--1685, 2009{\natexlab{b}}.

\bibitem[Vinyals et~al.(2017)Vinyals, Ewalds, Bartunov, Georgiev, Vezhnevets,
  Yeo, Makhzani, K{\"u}ttler, Agapiou, Schrittwieser, et~al.]{starcraft}
Vinyals, O., Ewalds, T., Bartunov, S., Georgiev, P., Vezhnevets, A.~S., Yeo,
  M., Makhzani, A., K{\"u}ttler, H., Agapiou, J., Schrittwieser, J., et~al.
\newblock Starcraft ii: A new challenge for reinforcement learning.
\newblock \emph{arXiv preprint arXiv:1708.04782}, 2017.

\bibitem[Zhao et~al.(2017)Zhao, Liu, Li, Li, and Du]{ngram2vec}
Zhao, Z., Liu, T., Li, S., Li, B., and Du, X.
\newblock Ngram2vec: Learning improved word representations from ngram
  co-occurrence statistics.
\newblock In \emph{Proceedings of the 2017 Conference on Empirical Methods in
  Natural Language Processing}, pp.\  244--253, 2017.

\end{thebibliography}

